Orthogonally Decoupled Variational Gaussian Processes

Gaussian processes (GPs) provide a powerful non-parametric framework for reasoning over functions. Despite appealing theory, its superlinear computational and memory complexities have presented a long-standing challenge. State-of-the-art sparse variational inference methods trade modeling accuracy against complexity. However, the complexities of these methods still scale superlinearly in the number of basis functions, implying that that sparse GP methods are able to learn from large datasets only when a small model is used. Recently, a decoupled approach was proposed that removes the unnecessary coupling between the complexities of modeling the mean and the covariance functions of a GP. It achieves a linear complexity in the number of mean parameters, so an expressive posterior mean function can be modeled. While promising, this approach suffers from optimization difficulties due to ill-conditioning and non-convexity. In this work, we propose an alternative decoupled parametrization. It adopts an orthogonal basis in the mean function to model the residues that cannot be learned by the standard coupled approach. Therefore, our method extends, rather than replaces, the coupled approach to achieve strictly better performance. This construction admits a straightforward natural gradient update rule, so the structure of the information manifold that is lost during decoupling can be leveraged to speed up learning. Empirically, our algorithm demonstrates significantly faster convergence in multiple experiments.

==> classification_table_acc.tex <==
\begin{tabular}{lllllllllll}
\toprule
                    &       N &   D &   K &             Selu & \textsc{Coupled} & \textsc{CoupledNat} &    \textsc{Orth} & \textsc{OrthNat} &  \textsc{Hybrid} & \textsc{Decoupled} \\
\midrule
              adult &   48842 &  15 &   2 &            84.76 &            85.85 &      \textbf{86.11} &            85.65 &   \textbf{86.15} &            85.73 &              84.37 \\
         chess-krvk &   28056 &   7 &  18 &   \textbf{88.05} &            67.38 &               60.23 &            67.76 &            60.70 &            59.34 &              53.56 \\
          connect-4 &   67557 &  43 &   2 &   \textbf{88.07} &            85.54 &               86.44 &            85.99 &            86.33 &            85.13 &              83.12 \\
             letter &   20000 &  17 &  26 &   \textbf{97.26} &            95.69 &               93.22 &            95.77 &            93.45 &            95.26 &              92.68 \\
              magic &   19020 &  11 &   2 &            86.92 &            89.24 &      \textbf{89.50} &            89.35 &   \textbf{89.42} &            89.19 &              88.33 \\
          miniboone &  130064 &  51 &   2 &            93.07 &            93.21 &      \textbf{93.60} &            93.49 &   \textbf{93.59} &            93.36 &              92.04 \\
           mushroom &    8124 &  22 &   2 &  \textbf{100.00} &  \textbf{100.00} &     \textbf{100.00} &  \textbf{100.00} &  \textbf{100.00} &  \textbf{100.00} &    \textbf{100.00} \\
            nursery &   12960 &   9 &   5 &   \textbf{99.78} &            97.30 &               97.30 &            97.30 &            97.30 &            97.30 &              97.29 \\
        page-blocks &    5473 &  11 &   5 &            95.83 &   \textbf{97.99} &               97.79 &            97.21 &            97.81 &            97.49 &              96.98 \\
          pendigits &   10992 &  17 &  10 &            97.06 &   \textbf{99.65} &      \textbf{99.64} &   \textbf{99.66} &   \textbf{99.64} &   \textbf{99.66} &     \textbf{99.62} \\
           ringnorm &    7400 &  21 &   2 &            97.51 &   \textbf{98.92} &               98.78 &            98.78 &            98.78 &   \textbf{98.86} &     \textbf{98.92} \\
    statlog-landsat &    6435 &  37 &   6 &            91.00 &            90.26 &      \textbf{91.45} &            91.28 &            91.08 &   \textbf{91.35} &              90.35 \\
    statlog-shuttle &   58000 &  10 &   7 &   \textbf{99.90} &   \textbf{99.87} &               99.74 &   \textbf{99.90} &   \textbf{99.81} &            99.79 &              99.80 \\
            thyroid &    7200 &  22 &   3 &            98.16 &            99.41 &      \textbf{99.56} &   \textbf{99.47} &            99.31 &   \textbf{99.52} &              99.13 \\
            twonorm &    7400 &  21 &   2 &   \textbf{98.05} &            97.67 &               97.65 &            97.65 &            97.72 &            97.69 &              97.72 \\
     wall-following &    5456 &  25 &   4 &            90.98 &            94.79 &               95.64 &            95.56 &   \textbf{95.76} &            93.07 &              91.48 \\
           waveform &    5000 &  22 &   3 &            84.80 &            85.80 &               86.54 &            86.13 &            86.21 &            86.53 &     \textbf{87.55} \\
     waveform-noise &    5000 &  41 &   3 &   \textbf{86.08} &            82.59 &               82.71 &            82.93 &            83.12 &            83.05 &              82.71 \\
 wine-quality-white &    4898 &  12 &   7 &   \textbf{63.73} &            57.14 &               58.61 &            57.05 &            59.56 &            56.58 &              55.71 \\
\midrule              Mean &         &     &     &             \textbf{91.6} &             90.4 &                90.2 &             90.6 &             90.3 &             89.9 &               89.0 \\
             Median &         &     &     &             93.1 &             94.8 &                93.6 &             \textbf{95.6} &             93.6 &             93.4 &               92.0 \\
           Avg Rank &         &     &     &             4.16 &             3.89 &                3.53 &             3.68 &             \textbf{3.42} &             3.89 &               5.42 \\
\bottomrule
\end{tabular}

==> classification_table_acc_summary.tex <==
\begin{tabular}{lccccccc}%
\toprule
                    &             Selu & \textsc{Coupled} & \textsc{CoupledNat} &    \textsc{Orth} & \textsc{OrthNat} &  \textsc{Hybrid} & \textsc{Decoupled} \\
\midrule              Mean &                    \textbf{91.6} &             90.4 &                90.2 &             90.6 &             90.3 &             89.9 &               89.0 \\
             Median &                    93.1 &             94.8 &                93.6 &             \textbf{95.6} &             93.6 &             93.4 &               92.0 \\
           Average rank &4.16(0.67)&	3.89(0.42)&	3.53(0.45)	&3.68(0.35)&	\textbf{3.42(0.31)}	&3.89(0.38)&	5.42(0.51) \\
           
\bottomrule
\end{tabular}

==> classification_table_lik.tex <==
\begin{tabular}{llllllllll}
\toprule
                    &       N &   D &   K &  \textsc{Coupled} & \textsc{CoupledNat} &     \textsc{Orth} &  \textsc{OrthNat} &   \textsc{Hybrid} & \textsc{Decoupled} \\
\midrule
              adult &   48842 &  15 &   2 &           -0.3048 &    \textbf{-0.2970} &           -0.3045 &  \textbf{-0.2973} &           -0.3067 &            -0.3234 \\
         chess-krvk &   28056 &   7 &  18 &  \textbf{-2.1239} &             -3.2821 &           -2.1625 &           -3.2145 &           -3.0443 &            -3.5380 \\
          connect-4 &   67557 &  43 &   2 &           -0.3160 &    \textbf{-0.3009} &           -0.3086 &  \textbf{-0.3017} &           -0.3244 &            -0.3680 \\
             letter &   20000 &  17 &  26 &           -0.2316 &             -0.4892 &  \textbf{-0.2276} &           -0.4793 &           -0.2810 &            -0.4861 \\
              magic &   19020 &  11 &   2 &           -0.2666 &    \textbf{-0.2641} &           -0.2658 &  \textbf{-0.2646} &           -0.2697 &            -0.2863 \\
          miniboone &  130064 &  51 &   2 &           -0.1680 &    \textbf{-0.1584} &           -0.1618 &  \textbf{-0.1585} &           -0.1645 &            -0.1902 \\
           mushroom &    8124 &  22 &   2 &  \textbf{-0.0006} &    \textbf{-0.0007} &  \textbf{-0.0009} &  \textbf{-0.0008} &  \textbf{-0.0007} &   \textbf{-0.0007} \\
            nursery &   12960 &   9 &   5 &  \textbf{-0.2228} &    \textbf{-0.2233} &  \textbf{-0.2225} &  \textbf{-0.2229} &           -0.2236 &            -0.2241 \\
        page-blocks &    5473 &  11 &   5 &           -0.1301 &    \textbf{-0.0989} &           -0.1328 &           -0.1112 &           -0.1368 &            -0.1538 \\
          pendigits &   10992 &  17 &  10 &           -0.0251 &    \textbf{-0.0216} &  \textbf{-0.0209} &  \textbf{-0.0207} &  \textbf{-0.0216} &            -0.0241 \\
           ringnorm &    7400 &  21 &   2 &  \textbf{-0.0345} &             -0.0458 &           -0.0466 &           -0.0465 &           -0.0410 &            -0.0418 \\
    statlog-landsat &    6435 &  37 &   6 &           -0.4503 &             -0.4102 &           -0.3956 &           -0.3920 &  \textbf{-0.3771} &            -0.4938 \\
    statlog-shuttle &   58000 &  10 &   7 &  \textbf{-0.0047} &             -0.0199 &  \textbf{-0.0049} &           -0.0174 &           -0.0170 &            -0.0166 \\
            thyroid &    7200 &  22 &   3 &           -0.0257 &             -0.0133 &  \textbf{-0.0115} &           -0.0211 &           -0.0127 &            -0.0290 \\
            twonorm &    7400 &  21 &   2 &  \textbf{-0.0590} &    \textbf{-0.0588} &  \textbf{-0.0590} &  \textbf{-0.0595} &           -0.0607 &            -0.0620 \\
     wall-following &    5456 &  25 &   4 &           -0.2032 &             -0.1674 &  \textbf{-0.1514} &           -0.1537 &           -0.3191 &            -0.4102 \\
           waveform &    5000 &  22 &   3 &           -0.6207 &             -0.5572 &           -0.5640 &  \textbf{-0.5038} &           -0.5160 &            -0.5469 \\
     waveform-noise &    5000 &  41 &   3 &           -0.7650 &             -0.7416 &           -0.7096 &  \textbf{-0.6778} &           -0.6893 &            -0.7673 \\
 wine-quality-white &    4898 &  12 &   7 &           -2.8884 &             -2.5400 &           -2.5681 &  \textbf{-2.5069} &           -2.7557 &            -2.7921 \\
\midrule               Mean &         &     &     &           -0.4653 &             -0.5100 &           \textbf{-0.4378} &           -0.4974 &           -0.5033 &            -0.5660 \\
             Median &         &     &     &            -0.223 &              -0.223 &            \textbf{-0.222} &            -0.223 &            -0.270 &             -0.286 \\
           Avg Rank &         &     &     &             3.553 &               3.026 &             2.868 &             \textbf{2.737} &             3.605 &              5.211 \\
\bottomrule
\end{tabular}

==> regression_table_lik.tex <==
\begin{tabular}{lllllllllll}
\toprule
                &        N &    D & \textsc{Coupled}$\dagger$ & \textsc{CoupledNat}$\dagger$ & \textsc{Coupled} & \textsc{CoupledNat} &  \textsc{OrthNat} & \textsc{Orth} & \textsc{Hybrid} & \textsc{Decoupled} \\
\midrule
         3droad &   434874 &    3 &                   -0.7630 &                      -0.7632 &          -0.7218 &             -0.7228 &  \textbf{-0.5947} &       -0.6103 &         -0.7617 &            -0.9438 \\
  houseelectric &  2049280 &   11 &                    1.3130 &                       1.3563 &           1.3383 &              1.3727 &   \textbf{1.3899} &        1.3719 &          1.3092 &             0.6032 \\
          slice &    53500 &  385 &                    0.7816 &                       0.7868 &           0.8321 &              0.8415 &   \textbf{0.8776} &        0.8701 &          0.7852 &             0.0655 \\
      elevators &    16599 &   18 &                   -0.4475 &                      -0.4455 &          -0.4448 &    \textbf{-0.4438} &           -0.4479 &       -0.4441 &         -0.4585 &            -0.4966 \\
           bike &    17379 &   17 &                    0.0059 &                       0.0135 &           0.0321 &     \textbf{0.0419} &            0.0271 &        0.0317 &         -0.0318 &            -0.1783 \\
   keggdirected &    48827 &   20 &                    1.0134 &                       1.0158 &           1.0214 &              1.0223 &   \textbf{1.0224} &        1.0216 &          1.0102 &             0.8947 \\
            pol &    15000 &   26 &                    0.0726 &                       0.0821 &           0.1047 &              0.1132 &   \textbf{0.1586} &        0.1451 &          0.0784 &            -0.2502 \\
 keggundirected &    63608 &   27 &                    0.6984 &                       0.6999 &           0.6994 &     \textbf{0.7020} &            0.7007 &        0.6967 &          0.6878 &             0.6374 \\
        protein &    45730 &    9 &                   -0.9531 &                      -0.9535 &          -0.9375 &             -0.9361 &  \textbf{-0.9138} &       -0.9165 &         -0.9527 &            -1.0464 \\
           song &   515345 &   90 &                   -1.1902 &                      -1.1898 &          -1.1890 &             -1.1884 &  \textbf{-1.1880} &       -1.1882 &         -1.1909 &            -1.2266 \\
           buzz &   583250 &   77 &                   -0.0566 &                      -0.0551 &          -0.0512 &             -0.0490 &  \textbf{-0.0480} &       -0.0484 &         -0.0614 &            -0.2285 \\
         kin40k &    40000 &    8 &                    0.0561 &                       0.1580 &           0.2191 &     \textbf{0.2234} &            0.1931 &        0.1777 &          0.1531 &            -0.3877 \\
           Mean &          &      &                    0.0442 &                       0.0588 &           0.0752 &              0.0814 &   \textbf{0.0981} &        0.0923 &          0.0472 &            -0.2131 \\
         Median &          &      &                     0.031 &                        0.048 &            0.068 &               0.078 &    \textbf{0.093} &         0.088 &           0.023 &             -0.239 \\
       Avg Rank &          &      &                     2.917 &                        4.000 &            5.417 &               6.750 &    \textbf{7.083} &         6.250 &           2.583 &              1.000 \\
\bottomrule
\end{tabular}




==> regression_table_lik_summary.tex <==
\begin{tabular}{lllllllllll}
\toprule
                &         \textsc{Coupled}$\dagger$ & \textsc{CoupledNat}$\dagger$ & \textsc{Coupled} & \textsc{CoupledNat} &  \textsc{OrthNat} & \textsc{Orth} & \textsc{Hybrid} & \textsc{Decoupled} \\
\midrule
           Mean &                          0.0442 &                       0.0588 &           0.0752 &              0.0814 &   \textbf{0.0981} &        0.0923 &          0.0472 &            -0.2131 \\
         Median &                          0.031 &                        0.048 &            0.068 &               0.078 &    \textbf{0.093} &         0.088 &           0.023 &             -0.239 \\
       Avg Rank & 2.917 &                        4.000 &            5.417 &               6.750 &    \textbf{7.083} &         6.250 &           2.583 &              1.000 \\
\bottomrule
\end{tabular}




==> regression_table_mae.tex <==
\begin{tabular}{lllllllllll}
\toprule
                &        N &    D & \textsc{Coupled}$\dagger$ & \textsc{CoupledNat}$\dagger$ & \textsc{Coupled} & \textsc{CoupledNat} & \textsc{OrthNat} &    \textsc{Orth} & \textsc{Hybrid} & \textsc{Decoupled} \\
\midrule
         3droad &   434874 &    3 &                    0.5160 &                       0.5163 &           0.4946 &              0.4951 &  \textbf{0.4332} &           0.4395 &          0.5150 &             0.6179 \\
  houseelectric &  2049280 &   11 &                    0.0632 &                       0.0604 &           0.0615 &              0.0595 &  \textbf{0.0583} &           0.0594 &          0.0636 &             0.1286 \\
          slice &    53500 &  385 &                    0.0840 &                       0.0837 &           0.0787 &              0.0779 &  \textbf{0.0730} &           0.0736 &          0.0838 &             0.2112 \\
      elevators &    16599 &   18 &                    0.3767 &                       0.3760 &           0.3756 &              0.3753 &           0.3770 &  \textbf{0.3752} &          0.3812 &             0.3973 \\
           bike &    17379 &   17 &                    0.2342 &                       0.2324 &           0.2283 &     \textbf{0.2261} &           0.2293 &           0.2282 &          0.2438 &             0.2848 \\
   keggdirected &    48827 &   20 &                    0.0883 &                       0.0878 &           0.0874 &     \textbf{0.0871} &           0.0871 &           0.0873 &          0.0883 &             0.0980 \\
            pol &    15000 &   26 &                    0.2073 &                       0.2058 &           0.2012 &              0.2000 &  \textbf{0.1906} &           0.1931 &          0.2065 &             0.2867 \\
 keggundirected &    63608 &   27 &                    0.1200 &                       0.1195 &           0.1197 &     \textbf{0.1191} &           0.1194 &           0.1202 &          0.1223 &             0.1304 \\
        protein &    45730 &    9 &                    0.6207 &                       0.6215 &           0.6118 &              0.6113 &  \textbf{0.5963} &           0.5972 &          0.6209 &             0.6868 \\
           song &   515345 &   90 &                    0.7954 &                       0.7951 &           0.7944 &              0.7939 &  \textbf{0.7936} &           0.7938 &          0.7960 &             0.8251 \\
           buzz &   583250 &   77 &                    0.2601 &                       0.2598 &           0.2586 &              0.2579 &  \textbf{0.2574} &           0.2576 &          0.2617 &             0.3106 \\
         kin40k &    40000 &    8 &                    0.2087 &                       0.1864 &           0.1768 &              0.1746 &  \textbf{0.1740} &           0.1776 &          0.1887 &             0.3501 \\
           Mean &          &      &                    0.2979 &                       0.2954 &           0.2907 &              0.2898 &  \textbf{0.2824} &           0.2836 &          0.2977 &             0.3606 \\
         Median &          &      &                     0.221 &                        0.219 &            0.215 &               0.213 &   \textbf{0.210} &            0.211 &           0.225 &              0.299 \\
       Avg Rank &          &      &                     6.083 &                        5.000 &            3.750 &               2.417 &   \textbf{1.833} &            2.500 &           6.417 &              8.000 \\
\bottomrule
\end{tabular}

==> regression_table_mae_summary.tex <==
\begin{tabular}{lccccccccc} %
\toprule
                &       \textsc{Coupled}$\dagger$ & \textsc{CoupledNat}$\dagger$ & \textsc{Coupled} & \textsc{CoupledNat} & \textsc{Orth} &    \textsc{OrthNat} & \textsc{Hybrid} & \textsc{Decoupled} \\
\midrule
           Mean &                           0.298 &                       0.295 &           0.291 &              0.290 &  0.284 &  \textbf{0.282} &                   0.298 &             0.361 \\
         Median &                           0.221 &                        0.219 &            0.215 &               0.213 &  0.211 &   \textbf{0.210} &                     0.225 &              0.299 \\
      Avg Rank &  6.083(0.19)&	5.00(0.33)&	3.750(0.26)&	2.417(0.31)&	2.500(0.47)&	\textbf{1.833(0.35)}&	6.417(0.23)&	8(0.00)\\
\bottomrule
\end{tabular}

==> regression_table_rmse.tex <==
\begin{tabular}{lllllllllll}
\toprule
                &        N &    D & \textsc{Coupled}$\dagger$ & \textsc{CoupledNat}$\dagger$ & \textsc{Coupled} & \textsc{CoupledNat} & \textsc{OrthNat} &    \textsc{Orth} & \textsc{Hybrid} & \textsc{Decoupled} \\
\midrule
         3droad &   434874 &    3 &                    0.5166 &                       0.5163 &           0.4946 &              0.4951 &  \textbf{0.4332} &           0.4395 &          0.6179 &             0.5150 \\
  houseelectric &  2049280 &   11 &                    0.0639 &                       0.0611 &           0.0615 &              0.0595 &  \textbf{0.0583} &           0.0594 &          0.1286 &             0.0636 \\
          slice &    53500 &  385 &                    0.0840 &                       0.0848 &           0.0787 &              0.0779 &  \textbf{0.0730} &           0.0736 &          0.2112 &             0.0838 \\
      elevators &    16599 &   18 &                    0.3767 &                       0.3760 &           0.3756 &              0.3753 &           0.3770 &  \textbf{0.3752} &          0.3973 &             0.3812 \\
           bike &    17379 &   17 &                    0.2342 &                       0.2324 &           0.2283 &     \textbf{0.2261} &           0.2293 &           0.2282 &          0.2848 &             0.2438 \\
   keggdirected &    48827 &   20 &                    0.0883 &                       0.0878 &           0.0874 &     \textbf{0.0871} &           0.0871 &           0.0873 &          0.0980 &             0.0883 \\
            pol &    15000 &   26 &                    0.2073 &                       0.2059 &           0.2012 &              0.2000 &  \textbf{0.1906} &           0.1931 &          0.2867 &             0.2065 \\
 keggundirected &    63608 &   27 &                    0.1200 &                       0.1196 &           0.1197 &     \textbf{0.1191} &           0.1194 &           0.1202 &          0.1304 &             0.1223 \\
        protein &    45730 &    9 &                    0.6207 &                       0.6216 &           0.6118 &              0.6113 &  \textbf{0.5963} &           0.5972 &          0.6868 &             0.6209 \\
           song &   515345 &   90 &                    0.7954 &                       0.7952 &           0.7944 &              0.7939 &  \textbf{0.7936} &           0.7938 &          0.8275 &             0.7960 \\
           buzz &   583250 &   77 &                    0.2601 &                       0.2606 &           0.2586 &              0.2579 &  \textbf{0.2574} &           0.2576 &          0.3106 &             0.2617 \\
         kin40k &    40000 &    8 &                    0.2087 &                       0.1885 &           0.1768 &              0.1746 &  \textbf{0.1740} &           0.1776 &          0.3501 &             0.1887 \\
\midrule
Mean &          &      &                    0.2980 &                       0.2958 &           0.2907 &              0.2898 &  \textbf{0.2824} &           0.2836 &          0.3608 &             0.2977 \\
         Median &          &      &                     0.221 &                        0.219 &            0.215 &               0.213 &   \textbf{0.210} &            0.211 &           0.299 &              0.225 \\
       Avg Rank &          &      &                     6.083 &                        5.167 &            3.750 &               2.417 &   \textbf{1.833} &            2.500 &           8.000 &              6.250 \\
\bottomrule
\end{tabular}
